Smells and Refactorings for Microservices Security: A Multivocal Literature Review

Context: Securing microservice-based applications is crucial, as many IT companies are delivering their businesses through microservices. If security smells affect microservice-based applications, they can possibly suffer from security leaks and need to be refactored to mitigate the effects of security smells therein. Objective: As the currently available knowledge on securing microservices is scattered across different pieces of white and grey literature, our objective here is to distill well-known smells for securing microservices, together with the refactorings enabling to mitigate the effects of such smells. Method: To capture the state of the art and practice in securing microservices, we conducted a multivocal review of the existing white and grey literature on the topic. We systematically analyzed 58 studies published from 2014 until the end of 2020. Results: Ten bad smells for securing microservices are identified, which we organized in a taxonomy, associating each smell with the security properties it may violate and the refactorings enabling to mitigate its effects. Conclusions: The security smells and the corresponding refactorings have pragmatic value for practitioners, who can exploit them in their daily work on securing microservices. They also serve as a starting point for researchers wishing to establish new research directions on securing microservices.

==> src/old/4-1-bad-practices.tex <==

\subsection{Trust the Network}
% describe security smell (when it happens, what it can result in)
A first, widely discussed bad practice is to \textsc{Trust the Network}, \viz designing microservices that blindly trust any other microservice from the same application.
This happens, \eg when no security is enforced in service-to-service communication, as the microservices of an application rely on network-level security. 
In the latter case, each microservice of an application is considered to be \enquote{trusted}, and whatever it claims about itself is trusted by the other microservices in the application \cite{25-Siriwardena-Microservices-Security-Action, 35-mody-zero-trust}. 
When this bad practice is followed, we may end up (in the worst case) with internal services blindly trusting whoever is calling them.
In such a scenario, an attacker compromising even a single microservice in an application would become able to manipulate all the other microservices in an application \cite{44-yarigina-security-challenges,45-esposito-challenges-cloud-microservices}.
% This may result, \eg in authenticity issues, as the attacker may start issuing arbitrary malicious requests to the microservices in an application, which the latter would fulfill as such request would be considered as coming from a trusted microservice \cite{44-yarigina-security-challenges,45-esposito-challenges-cloud-microservices}. 
% Confidentiality and integrity leaks may result as well, since the attacker may exploit the violated microservice to send requests to other microservices to read or manipulate the application data.

% describe refactoring
The authors of the 13 studies describing the \textsc{Trust the Network} bad practice all agree on saying that, to avoid incurring in such a bad practice, we should \textsc{Follow the Zero-Trust Principle}. 
The zero-trust approach assumes that the network is always hostile and untrusted, and it never takes anything for granted. 
Each request must be authenticated and authorized at each node before being accepted for further processing \cite{25-Siriwardena-Microservices-Security-Action}. 
Even if a request originates from a microservice at the same network-level, we should never assume that we can trust the source microservice and we should verify it based on what the credentials are \cite{14-Poddar-Webinar-Simplifying-Microservices-Security}. 
In other words, we should treat the microservices forming an application in the very same way as we would treat third-party applications \cite{36-parecki-oauth}.


\subsection{No Layered Security}
% describe security smell (when it happens, what it can result in)
Another bad practice is the so-called \textsc{No Layered Security}.
This occurs when we design microservice-based application to rely only on perimeter defense, or when we decide to adopt a single security solution or practice \cite{31-wallarm-shift-left}. 
Securing the perimeter or adopting a single security solution are not going to be enough, because microservices communicate with each other over the network and in disparate manners.
Each communication channel between any two microservices creates a potential attack vector that can be exploited by an intruder. 
Therefore, microservices-based applications call for a more robust defense involving multiple layers of security controls \cite{44-yarigina-security-challenges}.

% describe refactoring
The \textsc{No Layered Security} bad practice is discussed in 21 studies, whose authors point out that we can avoid incurring in such bad practice if we \textsc{Enact Defense in-Depth}. 
Defense-in-depth is a strategy in which several layers of security control are introduced in an application. 
We should protect critical services with multiple security layers, so a potential attacker who has exploited one of the microservices in our application may not be able to do so to other microservices or layers \cite{23-Kanjilal-4-fundamental-microservices-security-best-practices}. 
This helps slowing down attacks when one layer of security fails, or a vulnerability is identified.
The microservice architecture allows the diversification of security layers that development teams can adopt on each microservice \cite{58-oneill-microservice-security}. 
A layered security helps designing the application in such a way that each layer handles different types of attacks and repels an attacker at the outermost layer \cite{25-Siriwardena-Microservices-Security-Action}.


\subsection{Non-Proactive Security}
% describe security smell (when it happens, what it can result in)
Preventing exploits by intruders is only one part of securing a microservice-based application.
Proactive detection and reaction are another essential part \cite{11-Raible-Security-Patterns-for-Microservice-Architectures}. Though it is impossible to protect against all types of attacks, microservices must be provided with detection and prevention capabilities against, \eg credential-stuffing and credential abuse attacks as well as the capability to detect malicious botnet \cite{10-Chandramouli-Security-Strategies-for-Microservices}. 
Following a \textsc{Non-Proactive Security} approach is hence a bad practice while designing microservice-based applications, as it would bring to not include security mechanisms that allow to proactively detect and react to potential/actual attacks.

% describe refactoring
The \textsc{Non-Proactive Security} bad practice is discussed in 16 out of the 61 selected studies.
From such 16 studies, it emerges that we can enhance proactive security in microservice-based application if we \textsc{Use Attack Mitigation Techniques} and if we \textsc{Keep Third-Party Components Up to Date}. 
Concrete examples of attack mitigation techniques that we should use are web application firewalls (WAFs) \cite{09-WALLARM-A-CISO-GUIDE-TO-CLOUD-APPLICATION-SECURITY} and rate limiting \cite{37-smith-secure-apis}.
A WAF is an application firewall for HTTP applications applying protection rules to HTTP conversations \cite{48-jackson-go-microservices}.
A WAF can also monitor the volume of cache misses to proactively detect that, \eg an API gateway is constantly performing middle-tier service calls due to cache misses, which would suggest that the cache is potentially suffering a malicious attack \cite{34-behrens-starting-avalanche}.
WAFs can hence be used to provide instant protection against SQL injection, cross-site scripting, illegal resource access, remote code execution, remote file inclusion, and other OWASP Top-10 threats \cite{owasp2017}. 
We should also use rate-limiting API calls to mitigate distributed denial-of-service (DDoS) attacks and protecting the backend applications that process the API calls \cite{37-smith-secure-apis}. 
Rate limiting consists of counting how many requests a server is accepting in a period and rejecting new ones when a limit is reached. 
For example, if someone tries to attack an API with hundreds of gigabytes of username/password combinations, it could take a while for them to authenticate successfully.
If development teams can detect this type of attack, they can slow down the service and the attacker will likely go away  \cite{59-raible-11-patterns-security-microservices}.

We should also \textsc{Keep Third-Party Components Up to Date}, so that we include all the latest security patches for the third-party components we use in our applications \cite{11-Raible-Security-Patterns-for-Microservice-Architectures,48-jackson-go-microservices}. 
A scanning software can  be used on the source code repository to identify vulnerable dependencies. 
This type of scan should be enacted in any phase of the deployment pipeline, from the primary line of code to its released versions and new code contributions.


\subsection{Non-scalable security controls}
% describe security smell (when it happens, what it can result in)
% Microservices security best practices are not just about deploying the right technology. For microservices adoption to be successful, the development and operations teams should converge in line with the concept of DevOps, but they should also have a close relationship with security groups to understand security processes and how to mitigate security risks \cite{23-Kanjilal-4-fundamental-microservices-security-best-practices}. Also, while dealing with microservices, there can be several changes each day.
Microservices are typically deployed by adopting DevOps practices: continuous integration/continous deployment (CI/CD) pipelines are indeed typically enacted to distribute microservice-based applications and to keep them updated in production.
CI/CD pipelines are themselves a source of possible security issues, and (given their full automation) they need fully automated, scalable security controls.
Suppose that, \eg we plan to upgrade a microservice-based application by changing or adding functionalities to some of its microservices.
Without automation, we would be required to scan the added code and its integration with the existing code for vulnerabilities and weaknesses before we could deploy it \cite{33-sass-security-microservices}. 
This would go in contrast with the automation needs of CI/CD pipelines, hence resulting in what the authors of 15 of the selected studies consider the \textsc{Non-Scalable Security Controls} smell.
%They need to tie this into their continuous integration processes so that this is performed as part of the release process.

% describe refactoring
Development teams that want to mitigate the \textsc{Non-Scalable Security Controls} smell should \textsc{Use DevSecOps} and \textsc{Enact Continuous Security Testing} to mitigate its effects. 
On the one hand, DevSecOps helps in integrating security processes, principles, best practices, and tools early in the development lifecycle, thereby encouraging collaboration among security experts and business analysts, architects, and development and operations teams, thus making everyone accountable and responsible for building secured systems \cite{05-Krishnamurthy-Transition-to-Microservice-Architecture}.
On the other hand, automation is the key to integrating quality protection in a way that ensures quick feedback on the impact of new changes. 
Continuous, automated security testing in software development helps realizing the speed and flexibility needed in CI/CD pipelines, and it also ensures a faster recovery \cite{31-wallarm-shift-left}. 
Automated testing can create and update baselines before every release with OWASP Top 10 \cite{owasp2017} and advanced libraries that are informed by discovered abnormalities across clients. 
Through automation, developers can meet their responsibility to facilitate fast releases and quicker code fixes. 
It releases teams from the impracticality of safer, more homogeneous coding or heavy training \cite{31-wallarm-shift-left}.

==> src/old/4-bad-practices-refactorings.tex <==
\Cref{fig:taxonomy-bad-practices-refactorings} illustrates a taxonomy for security bad practices and for the refactorings allowing to mitigate them. We obtained this taxonomy following the same approach that we present in \Cref{sec:smells-refactorings}:

\begin{enumerate}
    \item We identified the bad practices by performing a first scan of the selected studies.
    
    \item We excerpted the refactorings directly from the selected studies after additional scans.
\end{enumerate}

The obtained security bad practices and refactorings were then manually organized to obtained a taxonomy. 
The taxonomy then underwent various iterations among the authors of this study, where corrections and amendments were applied to the taxonomy.
As a result, we obtained the final version of the taxonomy displayed in \Cref{fig:taxonomy-bad-practices-refactorings}, where the refactorings associated to a bad practice should \textit{all} be applied to mitigate its effects.

\begin{figure}
  \centering 
  \footnotesize
  \includegraphics[width=.9\textwidth]{figs/taxonomy-bad-practices-refactorings.pdf}
  \\
  \hfill (a) \hspace{5.7cm} (b) \hfill \ 
  \caption{Taxonomy of microservices security (a) bad practices and (b) refactorings.}
  \label{fig:taxonomy-bad-practices-refactorings}
\end{figure}

\Cref{tab:bad-practices-classification} shows the classification of all selected studies based on the taxonomy in \Cref{fig:taxonomy-bad-practices-refactorings}. 
The table provides a first overview of the coverage of the security bad practices over the selected studies. Such coverage is also displayed in the pie chart in \Cref{fig:coverage-bad-practices}, from which we can observe that all bad practices in the taxonomy are significantly recognized by the authors of the selected studies, hence making it worthy to discuss them in detail.
We hereafter present each security bad practice, together with the refactorings enabling to mitigate its possible effects. 

\input{tables/studies-and-bad-practices}

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth,trim=0 1.3cm 0 1.1cm]{data/bad-practices-bars.pdf}
    \caption{Coverage of the microservices security bad practices in the selected studies.}
    \label{fig:coverage-bad-practices}
\end{figure}

\input{src/4-1-bad-practices}

==> src/old/Old-3-taxonomy.tex <==
\Cref{fig:taxonomy-smells-refactorings} illustrates a taxonomy for the security smells pertaining to the considered security properties, and for the refactorings allowing to mitigate such smells. We obtained our taxonomy by following the guidelines for conducting systematic reviews in software engineering proposed by Petersen et al. \cite{Petersen2008}:

\begin{enumerate}
    \item We identified the security smells by performing a first scan of the selected studies.
    
    \item We excerpted the refactorings directly from the selected studies after additional scans.
\end{enumerate}

The obtinaed security smells and refactorings were then manually organized to obtained a taxonomy. 
A first version of the taxonomy was obtained by grouping the security smells based on the security properties they pertain to, by taking the security properties defined in the ISO/IEC 25010 standard \cite{ISO-standard} as a reference.
Out of the five properties defined in the ISO/IEC 25010, only three of them (\viz integrity, confidentiality, and authenticity) resulted to be directly corresponding to some of the identified security smells.  
All the security smells pertaining to more than one of ISO/IEC 25010 security properties were instead marked as \enquote{cross-cutting}.

\begin{figure}
  \centering 
  \footnotesize
  \includegraphics[width=.9\textwidth]{figs/taxonomy-smells-refactorings.pdf}
  \\
  \hfill (a) \hspace{4.6cm} (b) \hspace{5cm} (c) \hfill \hspace*{.5cm}
  \caption{Taxonomy of security (a) properties, (b) smells, and (c) refactorings.}
  \label{fig:taxonomy-smells-refactorings}
\end{figure}

\begin{figure}
  \centering 
  \footnotesize
  \includegraphics[width=.9\textwidth]{figs/taxonomy-bad-practices-refactorings.pdf}
  \\
  \hfill (a) \hspace{5.7cm} (b) \hfill \ 
  \caption{Taxonomy of security (a) bad practices and (b) refactorings.}
  \label{fig:taxonomy-bad-practices-refactorings}
\end{figure}

The taxonomy of security properties, smells, and refactorings underwent various iterations among the authors of this study. 
This resulted in some corrections and amendments to the first version of the taxonomy, which resulted in the final version of the taxonomy displayed in \Cref{fig:taxonomy-smells-refactorings}.




==> tables/old-studies-and-smells.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[p]
\centering
\caption{Classification of the selected studies according to the taxonomy in \Cref{fig:taxonomy-smells-refactorings}.}
\label{tab:classification}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
%   & \multicolumn{4}{c|}{integrity} & \multicolumn{3}{c|}{confidentiality} & \multicolumn{4}{c|}{authenticity} & \multicolumn{3}{c|}{cross-cutting} \\ \cline{2-15} 
 &
  \begin{tabular}[c]{@{}c@{}}own\\ crypto\\ code\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}sensitive\\ data\\ exposure\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}hardcoded\\ secrets\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}insecure\\ service\\ to service\\ comm.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non-proper \\ access \\ control\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}publicly \\ accessible \\ microserv.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}unneces. \\ privileges \\ to \\ microserv.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}unauth.\\ traffic\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}trust\\ the \\ network\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}central.\\ auth.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}decentr.\\ user\\ auth.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}no\\ layered \\ security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non\\ proactive\\ security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non\\ scalable\\ security \\ controls\end{tabular} \\ \hline
\cite{27-Abasi-Securing-modern-API-microservice} &        &       &       &       & \checkmark          & \checkmark          & \checkmark          & \checkmark      &        &        &        &            & \checkmark         &           \\ \hline
\cite{34-behrens-starting-avalanche} &        &       &       &       &            &            & \checkmark          &        &        &        & \checkmark      &            & \checkmark         &           \\ \hline
\cite{07-Boersma-Top-10-security-traps-to-avoid}  &        & \checkmark     &       & \checkmark     &            &            & \checkmark          & \checkmark      &        &        &        & \checkmark          & \checkmark         &           \\ \hline
\cite{51-bogner-microservices-industry} &        &       &       &       &            & \checkmark          &            &        &        &        &        &            &           &           \\ \hline
\cite{30-budko-5-things-api-security} &        &       &       &       &            &            &            & \checkmark      &        &        &        & \checkmark          &           &           \\ \hline
\cite{08-Carnell-Securing-your-microservices}  &        &       &       & \checkmark     & \checkmark          & \checkmark          & \checkmark          &        &        &        &        &            &           &           \\ \hline
\cite{10-Chandramouli-Security-Strategies-for-Microservices} &        &       &       & \checkmark     &            &            &            & \checkmark      &        &        & \checkmark      &            & \checkmark         &           \\ \hline
\cite{20-da-Silva-Best-Practices-to-Protect-Your-Microservices-Architecture} & \checkmark      & \checkmark     &       & \checkmark     &            &            & \checkmark          &        &        &        & \checkmark      &            & \checkmark         &           \\ \hline
\cite{28-Doerfeld-Control-user-identity-microservices} &        &       &       &       & \checkmark          &            &            & \checkmark      &        &        &        &            &           &           \\ \hline
\cite{32-douglas-microservice-authentication} &        &       &       & \checkmark     &            & \checkmark          &            &        &        & \checkmark      & \checkmark      &            &           &           \\ \hline
\cite{12-Edureka-Best-Practices-To-Secure-Microservices} &        &       &       & \checkmark     & \checkmark          &            &            &        &        &        & \checkmark      & \checkmark          &           &           \\ \hline
\cite{45-esposito-challenges-cloud-microservices} &        &       &       & \checkmark     &            &            &            &        & \checkmark      &        &        &            &           &           \\ \hline
\cite{18-Feitosa-Microservice-Patterns-and-Best-Practices} &        &       &       & \checkmark     &            & \checkmark          &            &        &        &        & \checkmark      &            &           &           \\ \hline
\cite{03-Gardner-Security-in-the-Microservices-Paradigm}  & \checkmark      &       &       &       &            & \checkmark          &            &        &        &        & \checkmark      &            &           &           \\ \hline
% \cite{41-gardner-security-microservices} & \checkmark      &       &       &       &            &            &            &        &        & \checkmark      & \checkmark      &            &           &           \\ \hline
\cite{38-gebel-securing-apis-microservices} &        &       &       &       & \checkmark          & \checkmark          &            & \checkmark      &        &        & \checkmark      &            &           &           \\ \hline
\cite{29-Gupta-security-strategies-devops} &        & \checkmark     &       & \checkmark     &            &            &            &        &        &        &        &            & \checkmark         & \checkmark         \\ \hline
\cite{17-Hofmann-Microservices-Best-Practices-for-Java} & \checkmark      & \checkmark     & \checkmark     &       & \checkmark          &            &            & \checkmark      & \checkmark      & \checkmark      & \checkmark      & \checkmark          &           & \checkmark         \\ \hline
\cite{46-indrasiri-microservices-security-fundamentals} &        &       &       & \checkmark     & \checkmark          & \checkmark          &            &        &        & \checkmark      & \checkmark      &            &           & \checkmark         \\ \hline
\cite{48-jackson-go-microservices} &        & \checkmark     &       & \checkmark     &            & \checkmark          & \checkmark          &        &        & \checkmark      & \checkmark      &            & \checkmark         &           \\ \hline
\cite{15-Jain-Top-10-Security-Best-Practices} &        & \checkmark     & \checkmark     & \checkmark     &            &            & \checkmark          &        &        &        &        & \checkmark          & \checkmark         &           \\ \hline
\cite{60-kamaruzzaman-microservice-architecture} &        &       &       &       &            & \checkmark          &            &        &        &        &        & \checkmark          &           &           \\ \hline
\cite{23-Kanjilal-4-fundamental-microservices-security-best-practices} &        &       &       & \checkmark     &            & \checkmark          & \checkmark          &        &        &        & \checkmark      & \checkmark          &           & \checkmark         \\ \hline
\cite{19-Khan-How-to-Secure-Your-Microservices} & \checkmark      &       & \checkmark     &       & \checkmark          & \checkmark          &            &        &        & \checkmark      &        &            &           &           \\ \hline
\cite{05-Krishnamurthy-Transition-to-Microservice-Architecture}  &        & \checkmark     &       &       & \checkmark          & \checkmark          &            &        &        &        &        & \checkmark          &           & \checkmark         \\ \hline
\cite{53-lea-microservice-security} &        &       &       & \checkmark     & \checkmark          &            & \checkmark          & \checkmark      & \checkmark      &        &        & \checkmark          &           &           \\ \hline
\cite{40-lemos-app-security} & \checkmark      &       &       & \checkmark     &            &            &            &        &        &        &        &            & \checkmark         & \checkmark         \\ \hline
\cite{02-Mannino-Security-In-The-Land-Of-Microservices}  &        &       & \checkmark     &       &            & \checkmark          &            &        &        & \checkmark      & \checkmark      &            &           &           \\ \hline
\cite{63-mateus-coehlo-security-microservices} &        & \checkmark     &       & \checkmark     &            &            &            &        &        &        & \checkmark      & \checkmark          &           &           \\ \hline
\cite{21-Matteson-10-tips-for-securing-microservice-architecture} &        &       &       & \checkmark     &            &            & \checkmark          &        &        &        &        &            &           & \checkmark         \\ \hline
\cite{24-Matteson-Establish-strong-microservices} &        &       &       & \checkmark     & \checkmark          & \checkmark          & \checkmark          &        & \checkmark      &        &        &            & \checkmark         &           \\ \hline
\cite{26-McLarty-Securing-Microservices-APIs} &        &       &       & \checkmark     & \checkmark          & \checkmark          &            & \checkmark      & \checkmark      & \checkmark      &        &            &           &           \\ \hline
\cite{35-mody-zero-trust} &        &       &       & \checkmark     &            &            & \checkmark          &        & \checkmark      &        &        &            &           &           \\ \hline
\cite{56-nehme-fine-grained-access-control} &        &       &       &       & \checkmark          & \checkmark          &            & \checkmark      &        & \checkmark      & \checkmark      &            &           &           \\ \hline
\cite{43-nehme-securing-microservices} &        &       &       &       & \checkmark          & \checkmark          &            &        &        & \checkmark      & \checkmark      &            & \checkmark         & \checkmark         \\ \hline
\cite{50-newman-building-microservices} & \checkmark      & \checkmark     &       &       &            &            &            &        & \checkmark      & \checkmark      &        & \checkmark          &           &           \\ \hline
\cite{13-Newman-Security-and-Microservices-by-Sam-Newman} &        & \checkmark     &       & \checkmark     & \checkmark          &            &            &        &        &        &        &            &           &           \\ \hline
\cite{55-nkomo-software-development-microservices} &        &       &       & \checkmark     &            &            &            & \checkmark      &        & \checkmark      & \checkmark      &            &           &           \\ \hline
\cite{58-oneill-microservice-security} & \checkmark      &       &       &       & \checkmark          & \checkmark          &            &        &        &        &        & \checkmark          &           & \checkmark         \\ \hline
\cite{36-parecki-oauth} &        &       & \checkmark     &       & \checkmark          &            &            &        & \checkmark      &        &        &            &           &           \\ \hline
\cite{39-perera-walking-the-wire} &        &       &       &       &            &            &            &        &        & \checkmark      &        &            &           &           \\ \hline
\cite{14-Poddar-Webinar-Simplifying-Microservices-Security} &        &       &       &       &            &            &            &        & \checkmark      &        &        &            &           &           \\ \hline
\cite{22-Radware-Microservice-Architectures-Challenge-Traditional-Security} &        &       &       & \checkmark     &            &            &            &        &        &        &        &            &           & \checkmark         \\ \hline
\cite{59-raible-11-patterns-security-microservices} &        &       & \checkmark     & \checkmark     & \checkmark          &            &            &        &        &        &        &            & \checkmark         & \checkmark         \\ \hline
% \cite{11-Raible-Security-Patterns-for-Microservice-Architectures} &        &       & \checkmark     & \checkmark     & \checkmark          &            &            & \checkmark      &        &        &        &            & \checkmark         &           \\ \hline
\cite{62-rajasekhariah-cloud-based-microservices} &        &       &       & \checkmark     &            & \checkmark          &            &        &        & \checkmark      &        &            &           &           \\ \hline
\cite{54-richter-security-microservices} &        &       &       &       &            &            &            &        &        & \checkmark      &        &            &           &           \\ \hline
\cite{06-Sahni-Best-Practices-for-Building-a-Microservice-Architecture}  & \checkmark      &       & \checkmark     &       &            &            &            & \checkmark      &        &        &        & \checkmark          &           & \checkmark         \\ \hline
\cite{33-sass-security-microservices} &        &       & \checkmark     & \checkmark     &            &            &            &        &        &        &        &            & \checkmark         & \checkmark         \\ \hline
\cite{47-sharma-mastering-microservices} &        &       &       & \checkmark     & \checkmark          &            &            &        &        &        &        &            &           &           \\ \hline
\cite{16-Siriwardena-Microservices-Security-Landscape} &        &       &       & \checkmark     &            & \checkmark          &            &        & \checkmark      &        &        &            &           &           \\ \hline
\cite{61-siriwardena-challenges-securing-microservices} &        &       &       &       &            &            &            &        & \checkmark      & \checkmark      &        &            &           &           \\ \hline
\cite{25-Siriwardena-Microservices-Security-Action} &        & \checkmark     &       & \checkmark     & \checkmark          & \checkmark          &            &        & \checkmark      & \checkmark      & \checkmark      & \checkmark          &           &           \\ \hline
\cite{42-smith-secure-microservices} &        &       &       &       &            & \checkmark          &            &        &        &        & \checkmark      &            &           &           \\ \hline
\cite{37-smith-secure-apis} &        & \checkmark     &       & \checkmark     & \checkmark          &            &            & \checkmark      &        &        & \checkmark      &            & \checkmark         &           \\ \hline
\cite{04-Sumo-Logic-Improving-Security-in-Your-Microservices-Architecture}  &        &       &       &       & \checkmark          & \checkmark          &            &        &        & \checkmark      &        & \checkmark          &           &           \\ \hline
\cite{57-torkura-cyber-risk-microservices} &        &       &       &       &            &            &            &        &        &        &        & \checkmark          &           &           \\ \hline
\cite{01-troisi-best-practices-microservices-app-security}  & \checkmark      &       &       &       & \checkmark          & \checkmark          &            &        &        &        &        & \checkmark          &           &           \\ \hline
\cite{09-WALLARM-A-CISO-GUIDE-TO-CLOUD-APPLICATION-SECURITY}  &        &       &       &       &            &            &            &        &        &        &        & \checkmark          & \checkmark         & \checkmark         \\ \hline
\cite{31-wallarm-shift-left} &        &       &       &       &            &            &            & \checkmark      &        &        &        & \checkmark          &           & \checkmark         \\ \hline
\cite{49-wolff-microservices-architecture} &        &       &       & \checkmark     & \checkmark          &            &            &        &        &        &        & \checkmark          &           &           \\ \hline
\cite{44-yarigina-security-challenges} &        &       &       & \checkmark     &            &            &            &        & \checkmark      & \checkmark      &        & \checkmark          &           &           \\ \hline
\cite{52-ziade-microservices-python} &        &       &       &       & \checkmark          &            &            &        &        & \checkmark      &        &            & \checkmark         &           \\ \hline
\end{tabular}%
}
\end{table}

==> tables/studies-and-bad-practices.tex <==
\begin{table}
\centering
\caption{Classification of the selected studies according to the taxonomy in \Cref{fig:taxonomy-bad-practices-refactorings}.}
\label{tab:bad-practices-classification}
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|}
\hline
 &
  \begin{tabular}[c]{@{}c@{}}trust the\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}no layered\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non proactive\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non scalable\end{tabular}\\
 &
  \begin{tabular}[c]{@{}c@{}}network\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security controls\end{tabular}\\ 
  \hline
\cite{27-Abasi-Securing-modern-API-microservice}&&&\checkmark&\\
\hline
\cite{34-behrens-starting-avalanche}&&&\checkmark&\\
\hline
\cite{07-Boersma-Top-10-security-traps-to-avoid}&&\checkmark&\checkmark&\\
\hline
\cite{51-bogner-microservices-industry}&&&&\\
\hline
\cite{30-budko-5-things-api-security} &
   &
  \checkmark &
   &
   \\ \hline
\cite{08-Carnell-Securing-your-microservices} &
   &
   &
   &
   \\ \hline
\cite{10-Chandramouli-Security-Strategies-for-Microservices} &
   &
   &
  \checkmark &
   \\ \hline
\cite{20-da-Silva-Best-Practices-to-Protect-Your-Microservices-Architecture} &
   &
   &
  \checkmark &
   \\ \hline
\cite{28-Doerfeld-Control-user-identity-microservices} &
   &
   &
   &
   \\ \hline
\cite{32-douglas-microservice-authentication} &
   &
   &
   &
   \\ \hline
\cite{12-Edureka-Best-Practices-To-Secure-Microservices} &
   &
  \checkmark &
   &
   \\ \hline
\cite{45-esposito-challenges-cloud-microservices} &
  \checkmark &
   &
   &
   \\ \hline
\cite{18-Feitosa-Microservice-Patterns-and-Best-Practices} &
   &
   &
   &
   \\ \hline
\cite{03-Gardner-Security-in-the-Microservices-Paradigm} &
   &
   &
   &
   \\ \hline
\cite{38-gebel-securing-apis-microservices} &
   &
   &
   &
   \\ \hline
\cite{29-Gupta-security-strategies-devops} &
   &
   &
  \checkmark &
  \checkmark \\ \hline
\cite{17-Hofmann-Microservices-Best-Practices-for-Java} &
  \checkmark &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{46-indrasiri-microservices-security-fundamentals} &
   &
   &
   &
  \checkmark \\ \hline
\cite{48-jackson-go-microservices} &
   &
   &
  \checkmark &
   \\ \hline
\cite{15-Jain-Top-10-Security-Best-Practices} &
   &
  \checkmark &
  \checkmark &
   \\ \hline
\cite{60-kamaruzzaman-microservice-architecture} &
   &
  \checkmark &
   &
   \\ \hline
\cite{23-Kanjilal-4-fundamental-microservices-security-best-practices} &
   &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{19-Khan-How-to-Secure-Your-Microservices} &
   &
   &
   &
   \\ \hline
\cite{05-Krishnamurthy-Transition-to-Microservice-Architecture} &
   &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{53-lea-microservice-security} &
  \checkmark &
  \checkmark &
   &
   \\ \hline
\cite{40-lemos-app-security} &
   &
   &
  \checkmark &
  \checkmark \\ \hline
\cite{02-Mannino-Security-In-The-Land-Of-Microservices} &
   &
   &
   &
   \\ \hline
\cite{63-mateus-coehlo-security-microservices} &
   &
  \checkmark &
   &
   \\ \hline
\cite{21-Matteson-10-tips-for-securing-microservice-architecture} &
   &
   &
   &
  \checkmark \\ \hline
\cite{24-Matteson-Establish-strong-microservices} &
  \checkmark &
   &
  \checkmark &
   \\ \hline
\cite{26-McLarty-Securing-Microservices-APIs} &
  \checkmark &
   &
   &
   \\ \hline
% \cite{35-mody-zero-trust} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{56-nehme-fine-grained-access-control} &
%   &
%   &
%   &
%   \\ \hline
% \cite{43-nehme-securing-microservices} &
%   &
%   &
%   \checkmark &
%   \checkmark \\ \hline
% \cite{50-newman-building-microservices} &
%   \checkmark &
%   \checkmark &
%   &
%   \\ \hline
% \cite{13-Newman-Security-and-Microservices-by-Sam-Newman} &
%   &
%   &
%   &
%   \\ \hline
% \cite{55-nkomo-software-development-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{58-oneill-microservice-security} &
%   &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{36-parecki-oauth} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{39-perera-walking-the-wire} &
%   &
%   &
%   &
%   \\ \hline
% \cite{14-Poddar-Webinar-Simplifying-Microservices-Security} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{22-Radware-Microservice-Architectures-Challenge-Traditional-Security} &
%   &
%   &
%   &
%   \checkmark \\ \hline
% \cite{59-raible-11-patterns-security-microservices} &
%   &
%   &
%   \checkmark &
%   \checkmark \\ \hline
% \cite{62-rajasekhariah-cloud-based-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{54-richter-security-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{06-Sahni-Best-Practices-for-Building-a-Microservice-Architecture} &
%   &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{33-sass-security-microservices} &
%   &&
%   \checkmark &
%   \checkmark \\ \hline
% \cite{47-sharma-mastering-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{16-Siriwardena-Microservices-Security-Landscape} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{61-siriwardena-challenges-securing-microservices} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{25-Siriwardena-Microservices-Security-Action} &
%   \checkmark &
%   \checkmark &
%   &
%   \\ \hline
% \cite{42-smith-secure-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{37-smith-secure-apis} &
%   &
%   &
%   \checkmark &
%   \\ \hline
% \cite{04-Sumo-Logic-Improving-Security-in-Your-Microservices-Architecture} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{57-torkura-cyber-risk-microservices} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{01-troisi-best-practices-microservices-app-security} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{09-WALLARM-A-CISO-GUIDE-TO-CLOUD-APPLICATION-SECURITY} &
%   &
%   \checkmark &
%   \checkmark &
%   \checkmark \\ \hline
% \cite{31-wallarm-shift-left} &
%   &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{49-wolff-microservices-architecture} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{44-yarigina-security-challenges} &
%   \checkmark &
%   \checkmark &
%   &
%   \\ \hline
% \cite{52-ziade-microservices-python}&&&\checkmark&\\ \hline
\end{tabular}%
\hspace{.5cm}
\begin{tabular}{|c|c|c|c|c|}
\hline
 &
  \begin{tabular}[c]{@{}c@{}}trust the\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}no layered\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non proactive\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}non scalable\end{tabular}\\
 &
  \begin{tabular}[c]{@{}c@{}}network\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}security controls\end{tabular}\\ 
  \hline
% \cite{27-Abasi-Securing-modern-API-microservice}&&&\checkmark&\\
% \hline
% \cite{34-behrens-starting-avalanche}&&&\checkmark&\\
% \hline
% \cite{07-Boersma-Top-10-security-traps-to-avoid}&&\checkmark&\checkmark&\\
% \hline
% \cite{51-bogner-microservices-industry}&&&&\\
% \hline
% \cite{30-budko-5-things-api-security} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{08-Carnell-Securing-your-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{10-Chandramouli-Security-Strategies-for-Microservices} &
%   &
%   &
%   \checkmark &
%   \\ \hline
% \cite{20-da-Silva-Best-Practices-to-Protect-Your-Microservices-Architecture} &
%   &
%   &
%   \checkmark &
%   \\ \hline
% \cite{28-Doerfeld-Control-user-identity-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{32-douglas-microservice-authentication} &
%   &
%   &
%   &
%   \\ \hline
% \cite{12-Edureka-Best-Practices-To-Secure-Microservices} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{45-esposito-challenges-cloud-microservices} &
%   \checkmark &
%   &
%   &
%   \\ \hline
% \cite{18-Feitosa-Microservice-Patterns-and-Best-Practices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{03-Gardner-Security-in-the-Microservices-Paradigm} &
%   &
%   &
%   &
%   \\ \hline
% \cite{38-gebel-securing-apis-microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{29-Gupta-security-strategies-devops} &
%   &
%   &
%   \checkmark &
%   \checkmark \\ \hline
% \cite{17-Hofmann-Microservices-Best-Practices-for-Java} &
%   \checkmark &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{46-indrasiri-microservices-security-fundamentals} &
%   &
%   &
%   &
%   \checkmark \\ \hline
% \cite{48-jackson-go-microservices} &
%   &
%   &
%   \checkmark &
%   \\ \hline
% \cite{15-Jain-Top-10-Security-Best-Practices} &
%   &
%   \checkmark &
%   \checkmark &
%   \\ \hline
% \cite{60-kamaruzzaman-microservice-architecture} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{23-Kanjilal-4-fundamental-microservices-security-best-practices} &
%   &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{19-Khan-How-to-Secure-Your-Microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{05-Krishnamurthy-Transition-to-Microservice-Architecture} &
%   &
%   \checkmark &
%   &
%   \checkmark \\ \hline
% \cite{53-lea-microservice-security} &
%   \checkmark &
%   \checkmark &
%   &
%   \\ \hline
% \cite{40-lemos-app-security} &
%   &
%   &
%   \checkmark &
%   \checkmark \\ \hline
% \cite{02-Mannino-Security-In-The-Land-Of-Microservices} &
%   &
%   &
%   &
%   \\ \hline
% \cite{63-mateus-coehlo-security-microservices} &
%   &
%   \checkmark &
%   &
%   \\ \hline
% \cite{21-Matteson-10-tips-for-securing-microservice-architecture} &
%   &
%   &
%   &
%   \checkmark \\ \hline
% \cite{24-Matteson-Establish-strong-microservices} &
%   \checkmark &
%   &
%   \checkmark &
%   \\ \hline
% \cite{26-McLarty-Securing-Microservices-APIs} &
%   \checkmark &
%   &
%   &
%   \\ \hline
\cite{35-mody-zero-trust} &
  \checkmark &
   &
   &
   \\ \hline
\cite{56-nehme-fine-grained-access-control} &
   &
   &
   &
   \\ \hline
\cite{43-nehme-securing-microservices} &
   &
   &
  \checkmark &
  \checkmark \\ \hline
\cite{50-newman-building-microservices} &
  \checkmark &
  \checkmark &
   &
   \\ \hline
\cite{13-Newman-Security-and-Microservices-by-Sam-Newman} &
   &
   &
   &
   \\ \hline
\cite{55-nkomo-software-development-microservices} &
   &
   &
   &
   \\ \hline
\cite{58-oneill-microservice-security} &
   &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{36-parecki-oauth} &
  \checkmark &
   &
   &
   \\ \hline
\cite{39-perera-walking-the-wire} &
   &
   &
   &
   \\ \hline
\cite{14-Poddar-Webinar-Simplifying-Microservices-Security} &
  \checkmark &
   &
   &
   \\ \hline
\cite{22-Radware-Microservice-Architectures-Challenge-Traditional-Security} &
   &
   &
   &
  \checkmark \\ \hline
\cite{59-raible-11-patterns-security-microservices} &
   &
   &
  \checkmark &
  \checkmark \\ \hline
\cite{62-rajasekhariah-cloud-based-microservices} &
   &
   &
   &
   \\ \hline
\cite{54-richter-security-microservices} &
   &
   &
   &
   \\ \hline
\cite{06-Sahni-Best-Practices-for-Building-a-Microservice-Architecture} &
   &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{33-sass-security-microservices} &
   &&
  \checkmark &
  \checkmark \\ \hline
\cite{47-sharma-mastering-microservices} &
   &
   &
   &
   \\ \hline
\cite{16-Siriwardena-Microservices-Security-Landscape} &
  \checkmark &
   &
   &
   \\ \hline
\cite{61-siriwardena-challenges-securing-microservices} &
  \checkmark &
   &
   &
   \\ \hline
\cite{25-Siriwardena-Microservices-Security-Action} &
  \checkmark &
  \checkmark &
   &
   \\ \hline
\cite{42-smith-secure-microservices} &
   &
   &
   &
   \\ \hline
\cite{37-smith-secure-apis} &
   &
   &
  \checkmark &
   \\ \hline
\cite{04-Sumo-Logic-Improving-Security-in-Your-Microservices-Architecture} &
   &
  \checkmark &
   &
   \\ \hline
\cite{57-torkura-cyber-risk-microservices} &
   &
  \checkmark &
   &
   \\ \hline
\cite{01-troisi-best-practices-microservices-app-security} &
   &
  \checkmark &
   &
   \\ \hline
\cite{09-WALLARM-A-CISO-GUIDE-TO-CLOUD-APPLICATION-SECURITY} &
   &
  \checkmark &
  \checkmark &
  \checkmark \\ \hline
\cite{31-wallarm-shift-left} &
   &
  \checkmark &
   &
  \checkmark \\ \hline
\cite{49-wolff-microservices-architecture} &
   &
  \checkmark &
   &
   \\ \hline
\cite{44-yarigina-security-challenges} &
  \checkmark &
  \checkmark &
   &
   \\ \hline
\cite{52-ziade-microservices-python}&&&\checkmark&\\ \hline
\multicolumn{5}{c}{}    \\
\end{tabular}%
\end{scriptsize}
\end{table}

